Enhancing Listened Speech Decoding from EEG via Parallel Phoneme Sequence Prediction

Brain-computer interfaces (BCI) offer numerous human-centered application possibilities, particularly affecting people with neurological disorders. Text or speech decoding from brain activities is a relevant domain that could augment the quality of life for people with impaired speech perception. We propose a novel approach to enhance listened speech decoding from electroencephalography (EEG) signals by utilizing an auxiliary phoneme predictor that simultaneously decodes textual phoneme sequences. The proposed model architecture consists of three main parts: EEG module, speech module, and phoneme predictor. The EEG module learns to properly represent EEG signals into EEG embeddings. The speech module generates speech waveforms from the EEG embeddings. The phoneme predictor outputs the decoded phoneme sequences in text modality. Our proposed approach allows users to obtain decoded listened speech from EEG signals in both modalities (speech waveforms and textual phoneme sequences) simultaneously, eliminating the need for a concatenated sequential pipeline for each modality. The proposed approach also outperforms previous methods in both modalities. The source code and speech samples are publicly available.

==> IEEEtranBST2/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> old/old.tex <==
% % Template for ICASSP-2024 paper; to be used with:
% %          spconf.sty  - ICASSP/ICIP LaTeX style file, and
% %          IEEEbib.bst - IEEE bibliography style file.
% % --------------------------------------------------------------------------
% \documentclass{article}
% \usepackage{spconf,amsmath,graphicx}
% \usepackage{booktabs}
% \usepackage{multirow,cite,bm}
% \usepackage{adjustbox}
% \usepackage{url}
% \usepackage{pifont}% http://ctan.org/pkg/pifont
% \newcommand{\cmark}{\ding{51}}%
% \newcommand{\xmark}{\ding{55}}%
% \usepackage[caption=false, position=top]{subfig}
% % Example definitions.
% % --------------------
% \def\x{{\mathbf x}}
% \def\L{{\cal L}}

% % Title.
% % ------
% \title{Enhancing Listened Speech Decoding from EEG Signals\\via Parallel Phoneme Prediction and Speech Synthesis}
% %
% % Single address.
% % ---------------
% \name{Jihwan Lee, Tiantian Feng, Aditya Kommineni, Sudarsana Reddy Kadiri, Shrikanth Narayanan}
% \address{University of Southern California, Los Angeles, USA}
% %
% % For example:
% % ------------
% %\address{School\\
% %	Department\\
% %	Address}
% %
% % Two addresses (uncomment and modify for two-address case).
% % ----------------------------------------------------------
% %\twoauthors
% %  {A. Author-one, B. Author-two\sthanks{Thanks to XYZ agency for funding.}}
% %	{School A-B\\
% %	Department A-B\\
% %	Address A-B}
% %  {C. Author-three, D. Author-four\sthanks{The fourth author performed the work
% %	while at ...}}
% %	{School C-D\\
% %	Department C-D\\
% %	Address C-D}
% %
% \begin{document}
% %\ninept
% %
% \maketitle
% %
% \begin{abstract}
% Brain-computer interfaces (BCI) hold tremendous promise for numerous human-centered applications, especially serving those with communication disorders.
% We propose a novel approach to enhance listened-speech decoding from electroencephalography (EEG) signals by utilizing an auxiliary phoneme predictor that decodes phoneme sequences simultaneously.
% The proposed model architecture mainly consists of three parts: an EEG module, a speech module, and a phoneme predictor.
% The EEG module learns to represent EEG signals into EEG embedding.
% The speech module generates speech waveforms from the EEG embeddings.
% The phoneme predictor outputs the decoded phonemes in text modality.
% Our proposed approach allows users to obtain decoded speech from EEG signals in both modalities simultaneously: acoustic speech waveforms and phoneme sequences, eliminating the need for a concatenated sequential pipeline for each modality. 
% The proposed approach also outperforms previous methods in both modalities.
% The source code and speech samples are available here: \url{link to github}

% \end{abstract}
% %
% \begin{keywords}
% One, two, three, four, five
% \end{keywords}
% %
% \section{Introduction}
% \label{sec:intro}

% Brain-computer interfaces (BCI) offer a promising avenue for a wide range of applications, particularly in assisting individuals with profound communication disorders.
% The ability to decode perceived, imagined or produced speech, as well as the corresponding text, from brain signals is fundamental to the development and effectiveness of these technologies.
% The successful integration of speech and text decoding into BCI leads to significant advances in neurorehabilitation, offering alternative communication means.

% Several 
% Two types of signal - invasive and non-invasive
% % Aditya to fill up EEG SSL paragraph 
% \par 
% Recently, there has been a growing interest to leverage self supervision to learn meaningful representations for biosignals, especially in EEG, with focus on generalizability of the pre-trained models to downstream tasks\cite{kommineni2024knowledgeguided, kostas2021bendr}(Maybe add one or two more?). Owing to EEG being inherently noisy, 
% EEG is challenging, introduce some recent ssl based eeg approaches.

% Approaches with text decoding

% speech decoding
% Recently a framework for direct reconstruction of listened speech waveforms has been proposed \cite{fesde}. 

% There are instances where the need arises to decode both speech and text from brain signals at the same time.
% However, most existing approaches are limited to only a single modality at a time.
% Consequently, to achieve decoding in both modalities, it is necessary to implement a concatenated, sequential pipeline, such as an additional speech synthesizer or recognizer.
% % Hence, a concatenated, sequential pipeline followed by an additional speech synthesizer or speech recognizer is required to acquire decoded speech in both modalities.
% % and the sequential decoding of the other followed by, such as an additional speech synthesizer followed by decoded text, or a speech recognizer followed by decoded speech.

% We propose a novel framework that can decode listened speech in both modalities (speech waveform and textual phonemes) simultaneously by utilizing an auxiliary phoneme predictor.
% The proposed framework utilizes an auxiliary phoneme predictor 

% Our main contributions are:
% \begin{itemize}
% \item We propose to utilize an auxiliary phoneme predictor to enhance listened speech decoding performance from EEG signals, outperforming previous apporaches.
% \item Our proposed framework allows parallel decoding of speech waveforms and textual phonemes from EEG signals. To our knowledge, this is the first approach.
% \item We provide the model characteristics of decoded phonemes and speech.
% \end{itemize}

% \section{Proposed Method}

% \subsection{Model Architecture}
% Our proposed framework consists of three major parts: the phoneme predictor, EEG module, and speech module.
% The EEG module learns the latent representation embeddings from EEG signals.
% The EEG embeddings are fed into the phoneme predictor and the speech module in parallel to output the predicted phonemes and decoded speech waveforms corresponding to given EEG signals, respectively.
% Note that our approach enables parallel decoding of both speech and textual phoneme at the same time, rather than sequentially concatenated pipeline of each modality.

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\linewidth]{figures/overall_archi_4.pdf}
%   \caption{The overall architecture of our proposed framework.}
%   \label{fig:overall-archi}
% \end{figure}

% \subsubsection{EEG and Speech Module}
% We adopt the EEG and speech module from \cite{fesde}.
% The EEG module learns to better represent input EEG signals to EEG embeddings.
% The speech modules learns to generate speech waveform from EEG embeddings, similar to \cite{fesde, vits}.
% It consists of speech encoder and speech decoder.
% There is a gradient stop between the EEG module and the speech module, hence the training of the EEG module is not influenced by the speech module.

% \subsubsection{Phoneme Predictor}
% The phoneme predictor consists of conformer blocks \cite{conformer} followed by a decoder made of an LSTM layer with an attention layer, as this is a well known approach in the automatic speech recognition (ASR) domain.
% The phoneme predictor takes the EEG embeddings as input then outputs the predicted phonemes.
% By doing so, the EEG embeddings contains better the phoneme information.




% % \input{tables/table-compare-models}

% \subsection{Training Objectives}
% We use the connectionist temporal classification (CTC) loss \cite{ctc-loss} for the phoneme predictor. The CTC loss is commonly used in the ASR domain, as it handles well with many-to-one mapping sequence decoding.
% We use the reconstruction loss for EEG identical to \cite{fesde, kommineni2024knowledgeguided}, as defined in Eq.~(\ref{equation:loss-cossim}):
% \begin{align}
% L_{\text{EEG}}(x, \hat{x}) = 1 - \frac{1}{N_{\text{ch}}}\sum_{i=1}^{N_{\text{ch}}}\frac{x_i^T \cdot \hat{x_i}}{\Vert x_i \Vert \Vert \hat{x_i}\Vert}
%   \label{equation:loss-cossim}
% \end{align}
% where $N_{\text{ch}}$ is the number of EEG channels ($N_{\text{ch}}=128$), and $x_i$ and $\hat{x_i}$ are $i\textsuperscript{th}$ channel of the input and the reconstructed EEG signals, respectively.
% The total training objective of the phoneme predictor and the EEG module is as in Eq.(\ref{equation:loss-pheeg}):
% \begin{align}
% L=L_{\text{EEG}} + \alpha L_{\text{ctc}}
% \label{equation:loss-pheeg}
% \end{align}
% We heuristically chose $\alpha=0.3$.
% We adopt the training objectives for the speech module from \cite{fesde,vits}, which consist of the mel-spectrogram reconstruction loss, the KL divergence loss between the latent representations of EEG and speech, and the GAN loss for the speech waveform generation. 
% A separate optimizer was used to train the speech module, as the stop gradient is applied between the EEG module and the speech module.

% % \input{tables/table-speech}
% % \input{tables/table-phoneme}


% \section{Experiments}
% \subsection{Dataset}
% Adopting the experimental setup in \cite{fesde}, we conducted our experiments on the N400 dataset \cite{n400}.
% The 128-channel EEG signals were collected from 24 subjects at a sampling rate of 512 Hz. Each subject listened to 440 synthesized, gender-neutral speech utterances in English.
% We chose two subjects and 40 sentences as held-out test sets, yielding three test sets: \texttt{unseen speech}, \texttt{unseen subject}, and \texttt{unseen both}.
% In the \texttt{unseen speech} or \texttt{unseen subject} test set, only the speech sentences or the subjects are held-out, respectively. In the \texttt{unseen both} test set, both speech sentences and subjects are held-out.
% % There are three test sets, unseen speech, unseen

% We employ the same pre-processing pipeline for the EEG signals as in \cite{fesde}: powerline removal (a 60 Hz notch filter), EEG spectral information preservation (a bandpass filter with low of 0.5 Hz and high 50 Hz), eye blink removal (independent component analysis), then downsample to 256 Hz.
% The speech samples were resampled to 22,050 Hz, which is the original sampling rate \cite{vits} had been designed for.
% We use \texttt{espeak G2P}\footnote{\url{https://github.com/espeak-ng/espeak-ng}} to convert the raw text(graphemes) to phonemes.

% \subsection{Experimental Setup}

% We compare three different configurations of our proposed framework. In \textsc{1-CB} and \textsc{2-CB}, one and two conformer blocks are used in the phoneme predictor, respectively. In \textsc{0-CB}, no conformer block is used, instead, only a single LSTM layer is used.

% We compare our model with two baselines, one for each speech and textual phoneme modality: \textsc{FESDE} \cite{fesde} for speech and \textsc{EEG2Text} \cite{eeg2text} for textual phoneme decoding.
% A few modifications have been made to \textsc{EEG2Text} to better adjust to our task. The pre-trained language model was removed as the pre-trained language model had been trained to predict text tokens, rather than phonemes. The single layer LSTM decoder identical to our proposed phoneme predictor has been utilized, instead.
% Two configurations of \textsc{EEG2Text} have been compared to our approach: \textsc{EEG2Text-sc} being trained from scratch without any pre-trained initial parameter weights; and \textsc{EEG2Text-pt} being pre-trained with EEG input only first then for the phoneme prediction task. In \textsc{EEG2Text-pt}, the identical EEG reconstruction loss as in our proposed approach was applied. % rather than the mask prediction loss. in order to minimize the number of different factors for more simple comparison.


% \begin{figure*}[!ht]
%   \centering
%   \subfloat[MCD (dB) of each consonant (bluish) and vowel (reddish) group.]{%
%   \includegraphics[clip, width=0.98\textwidth,height=3.9cm]{figures/together_err_mcd.pdf}%
%   }
%   \vspace{-3mm}

%   \subfloat[Mel-Corr (\%) of each consonant (bluish) and vowel (reddish) group.]{%
%   \includegraphics[clip, width=0.98\textwidth,height=3.9cm]{figures/together_err_melcorr.pdf}%
%   }

%   \vspace{-3mm}

%   \subfloat[Top 3 Accuracy (\%) of each consonant (blue) and vowel (red) group.]{%
%   \includegraphics[clip, width=0.98\textwidth,height=3.9cm]{figures/top3_preds.pdf}%
%   \label{fig:phonemes-top3}
%   }

%   \vspace{-3mm}

%     \caption{MCD (dB), Mel-Corr (\%), and Top-3 accuracy (\%) of each phoneme group with respect to the number of the conformer blocks. The lower MCD and higher Mel-Corr and top-3 accuracy indicate better performance. The consonants (blue) are clustered by three criteria: manner, place, and voicedness of articulation. The vowels (red) are clustered by its tongue position and tenseness.}
%   \label{fig:phonemes}
% \end{figure*}

% \section{Results and Discussion}
% \subsection{Evaluation on Speech Decoding}
% We evaluate our results on two criteria: speech and textual phoneme. 
% For speech, we adopt the evaluation measures as in \cite{fesde}: mel cepstral distortion (MCD) \cite{mcd} and the Pearson correlation between two mel-spectrograms (Mel-Corr). MCD is the Eucleadian distance between two mel-cepstral coefficients as defined in Eq~(\ref{equation:mcd}):
% \begin{align}
% \vspace{-0.5cm}
% \text{MCD} = \frac{10\sqrt{2}}{\ln10}\sqrt{\sum_{i=1}^{N_\text{MCC}}(\text{MCC}_i-\widehat{\text{MCC}_i})^2}
%   \label{equation:mcd}
%   \vspace{-0.5cm}
% \end{align}
% Lower MCD and higher Mel-Corr values represent the higher quality of decoded speech waveforms. For simpler notation, the Mel-Corr values are multiplied by 100.
% As shown in Table~\ref{tab:mcd-corr}, all of our training configurations outperform the baseline \cite{fesde} in both metrics.
% Our proposed approach achieves a great improvement, especially in terms of Mel-Corr, doubling the metrics.
% The best performance is observed when a single LSTM layer was utilized as the phoneme predictor.

% \subsection{Evaluation on Textual Phoneme Decoding}
% For textual phonemes, we adopt top-k accuracy of subsequent phoneme prediction given EEG signals and previous phoneme inputs, similar to \cite{meta-paper}.
% We find the top-k accuracy more reliable than the raw phoneme error rates (PER), as there is no error correction made by any external language model in our experimental setup, initial errors often leading to huge error accumulation.
% % We show 
% % As there is no error correction made by any external language model in our experimental setup, we find the raw phoneme error rates (PER), as initial error often leads to huge error accumulation.
% % We also did not use BLUE or ROUGH scores, as they are more suitable where multiple references are available, which is not the case here.
% As shown in Table~\ref{tab:topk}, our proposed approach outperforms the both of the training configurations of the baseline \cite{eeg2text}, when two conformer blocks are used in the phoneme predictor.
% The exceptionally high accuracy in the unseen subject test set may occur due to overfitting, as the target phoneme sequences are already seen during training in this split.

% \subsection{Effects of Conformer}

% We observe a trade-off between the performances on each modality with respect to the number of the conformer blocks used in the phoneme predictor.
% The speech decodability tends to decrease when more conformer blocks are used, while the textual phoneme decodability shows the opposite tendency.
% Note that the speech decoding still outperforms the baseline \cite{fesde} even in our worst performing configuration.
% We analyze deeper into the characteristics of the phonemes where this performance trade-off happens in the subsequent Section~\ref{sec:phoneme-analysis}.

% \subsection{Analysis on Phoneme Groups}
% \label{sec:phoneme-analysis}
% In this section, we address the following questions: identify specific phoneme groups that perform poorly/well on each modality 1) in general; and 2) with respect to the number of the conformer blocks.
% Figure~\ref{fig:phonemes} depicts the decodabilty of each phoneme group, with respect to the number of conformer blocks. The identical analysis pipeline was utilized as in \cite{fesde}. The unseen subject test set is excluded from the top-3 accuracy analysis in Figure~\ref{fig:phonemes-top3}, as the text is seen during training and it shows different tendency compared to the other test sets.
% We observe the performance trade-off occurs in the consonants more dominantly than the vowels.
% In the speech-wise, the performance drop mostly occurs 











% % \section{Ablation Study}
% % \subsection{EEG Pre-training}
% % Contrary to \cite{fesde,eeg2text}, we observe performance drop in our proposed framework, when the EEG module is initialized with pre-trained parameter weights.


% \section{Conclusion and Future Work}
% We propose to the framework to decode listened speech from EEG signals utilizing an auxiliary phoneme predictor, enhancing its performance in both speech and textual phoneme decoding.
% The proposed framework enables parallel decoding of both speech and textual phonemes, hence, concatenated, sequential pipeline of each modality decoder is no longer necessary.

% We look forward to expand our work to speech production tasks, such as decoding phonated, attempted, or imagined speech from neural activities, as current work is limited to the speech perception task.
% We also plan to further improve the performance by leveraging pre-trained models for each modality.





% % Below is an example of how to insert images. Delete the ``\vspace'' line,
% % uncomment the preceding line ``\centerline...'' and replace ``imageX.ps''
% % with a suitable PostScript file name.
% % -------------------------------------------------------------------------


% % To start a new column (but not a new page) and help balance the last-page
% % column length use \vfill\pagebreak.
% % -------------------------------------------------------------------------
% %\vfill
% %\pagebreak



% % References should be produced using the bibtex program from suitable
% % BiBTeX files (here: strings, refs, manuals). The IEEEbib.bst bibliography
% % style file from IEEE produces unsorted bibliography list.
% % -------------------------------------------------------------------------
% % \small
% \clearpage
% \small
% \bibliographystyle{IEEEbib}
% \bibliography{strings,refs}

% \end{document}

